Knowledge Distillation for Multi-Target Domain Adaptation in Real-Time Person Re-Identification

Despite the recent success of deep learning architectures, person re-identification (ReID) remains a challenging problem in real-word applications. Several unsupervised single-target domain adaptation (STDA) methods have recently been proposed to limit the decline in ReID accuracy caused by the domain shift that typically occurs between source and target video data. Given the multimodal nature of person ReID data (due to variations across camera viewpoints and capture conditions), training a common CNN backbone to address domain shifts across multiple target domains, can provide an efficient solution for real-time ReID applications. Although multi-target domain adaptation (MTDA) has not been widely addressed in the ReID literature, a straightforward approach consists in blending different target datasets, and performing STDA on the mixture to train a common CNN. However, this approach may lead to poor generalization, especially when blending a growing number of distinct target domains to train a smaller CNN. To alleviate this problem, we introduce a new MTDA method based on knowledge distillation (KD-ReID) that is suitable for real-time person ReID applications. Our method adapts a common lightweight student backbone CNN over the target domains by alternatively distilling from multiple specialized teacher CNNs, each one adapted on data from a specific target domain. Extensive experiments conducted on several challenging person ReID datasets indicate that our approach outperforms state-of-art methods for MTDA, including blending methods, particularly when training a compact CNN backbone like OSNet. Results suggest that our flexible MTDA approach can be employed to design cost-effective ReID systems for real-time video surveillance applications.

==> temp_bib <==
@inproceedings{ristani2016performance,
  title={Performance measures and a data set for multi-target, multi-camera tracking},
  author={Ristani, E. and Solera, F. and Zou, R. and Cucchiara, R. and Tomasi, C.},
  booktitle={ECCV 2016}
}


@inproceedings{loss_ces,
  title={Rethinking the inception architecture for computer vision},
  author={Szegedy, C. and Vanhoucke, V. and Ioffe, S. and Shlens, J. and Wojna, Z.},
  booktitle={ICCV 2016}
}
@article{hermans2017defense,
  title={In defense of the triplet loss for person reID},
  author={Hermans, A. and Beyer, L. and Leibe, B.},
  journal={arXiv 2017},
}
@article{gretton2012kernel,
  title={A kernel two-sample test},
  author={Gretton, A. and Borgwardt, K. M and Rasch, M. and Sch{\"o}lkopf, B. and Smola, A.},
  journal={Journal of MLR},
  volume={13},
  number={1},
  pages={723--773},
  year={2012},
}

@inproceedings{heo2019overhaul,
title={A comprehensive overhaul of feature distillation},
author={Heo, B. and Kim, J. and Yun, S. and Park, H. and Kwak, N. and Choi, J.},
booktitle={ICCV 2019}
}

@article{wang2021knowledge,
  title={Knowledge distillation and student-teacher learning for visual intelligence: A review and new outlooks},
  author={Wang, L. and Yoon, K},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2021},
 }

@article{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, G. and Vinyals, O. and Dean, J.},
  journal={arXiv 2015}
}

@inproceedings{mekhazni2020unsupervised,
  title={Unsupervised DA in the dissimilarity space for person reID},
  author={Mekhazni, D. and Bhuiyan, A. and Ekladious, G. and Granger, E.},
  booktitle={ECCV 2020}
  }

@article{NGUYENMEIDINE2021104096,
    title = {Knowledge distillation methods for efficient unsupervised adaptation across multiple domains},
    author = {L.T. Nguyen-Meidine and A. Belal and M. Kiran and J. Dolz and L. A. Blais-Morin and E. Granger}
    journal={Image and Vision Computing},
    volume={108},
    year={2021}
}

@inproceedings{luo2019bag,
  title={Bag of tricks and a strong baseline for deep person reID},
  author={Luo, H. and Gu, Y. and Liao, X. and Lai, S. and Jiang, W.},
  booktitle={CVPR Workshops 2019},
}

@inproceedings{quan2019auto,
  title={Auto-reid: Searching for a part-aware convnet for person reID},
  author={Quan, R. and Dong, X. and Wu, Y. and Zhu, L. and Yang, Y.},
  booktitle={ICCV 2019}
}

@inproceedings{wang2019spatial,
  title={Spatial-temporal person reID},
  author={Wang, G. and Lai, J. and Huang, P. and Xie, X.},
  booktitle={AAAI 2019}
}

@article{nguyen2020joint_DA,
  title={Joint progressive knowledge distillation and unsupervised DA},
  author={Nguyen-Meidine, L.T. and Granger, E. and Kiran, M. and Dolz, J. and Blais-Morin, L.A.},
  journal={arXiv 2020},
}

@article{wang2018deep_DA,
  title={Deep visual DA: A survey},
  author={Wang, M. and Deng, W.},
  journal={Neurocomputing},
  volume={312},
  pages={135--153},
  year={2018}
}

@inproceedings{wang2016joint,
  title={Joint learning of single-image and cross-image representations for person reID},
  author={Wang, F. and Zuo, W. and Lin, L. and Zhang, D. and Zhang, L.},
  booktitle={CVPR 2016}
}

@inproceedings{cheng2016person,
  title={Person reID by multi-channel parts-based cnn with improved triplet loss function},
  author={Cheng, D. and Gong, Y. and Zhou, S. and Wang, J. and Zheng, N.},
  booktitle={CVPR 2016}
}

@inproceedings{shi2016embedding,
  title={Embedding deep metric for person reID: A study against large variations},
  author={Shi, H. and Yang, Y. and Zhu, X. and Liao, S. and Lei, Z. and Zheng, W. and Li, S.Z.},
  booktitle={ECCV 2016}
}

@article{geng2016deep,
  title={Deep transfer learning for person reID},
  author={Geng, M. and Wang, Y. and Xiang, T. and Tian, Y.},
  journal={arXiv 2016}
}

@article{zheng2017discriminatively,
  title={A discriminatively learned cnn embedding for person reidentification},
  author={Zheng, Z. and Zheng, L. and Yang, Y.},
  journal={ACM Transactions on Multimedia Computing, Communications, and Applications},
  volume={14},
  number={1},
  pages={1--20},
  year={2017},
}

@article{zhang2018learning,
  title={Learning compact appearance representation for video-based person reID},
  author={Zhang, W. and Hu, S. and Liu, K. and Zha, Z.},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  volume={29},
  number={8},
  pages={2442--2452},
  year={2018},
}

@inproceedings{zheng2017unlabeled,
  title={Unlabeled samples generated by gan improve the person reID baseline in vitro},
  author={Zheng, Z. and Zheng, L. and Yang, Y.},
  booktitle={ICCV 2017}
}

@inproceedings{schroff2015facenet,
  title={Facenet: A unified embedding for face recognition and clustering},
  author={Schroff, F. and Kalenichenko, D. and Philbin, J.},
  booktitle={CVPR 2015}
}

@article{weinberger2009distance,
  title={Distance metric learning for large margin nearest neighbor classification},
  author={Weinberger, K. and Saul, L.},
  journal={J. of Machine Learning Research},
  volume={10},
  pages = {207--244},
  number={2},
  year={2009}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, K. and Zhang, X. and Ren, S. and Sun, J.},
  booktitle={CVPR 2016}
}

@inproceedings{heo2019comprehensive,
  title={A comprehensive overhaul of feature distillation},
  author={Heo, B. and Kim, J. and Yun, S. and Park, H. and Kwak, N. and Choi, J.Y.},
  booktitle={ICCV 2019}
}

@inproceedings{mirzadeh2020improved,
  title={Improved knowledge distillation via teacher assistant},
  author={Mirzadeh, S.I. and Farajtabar, M. and Li, A. and Levine, N. and Matsukawa, A. and Ghasemzadeh, H.},
  booktitle={AAAI 2020}
}

@inproceedings{ganin2015unsupervised,
  title={Unsupervised DA by backpropagation},
  author={Ganin, Y. and Lempitsky, V.},
  booktitle={ICML 2015}
}

@inproceedings{tzeng2017adversarial,
  title={Adversarial discriminative DA},
  author={Tzeng, E. and Hoffman, J. and Saenko, K. and Darrell, T.},
  booktitle={CVPR 2017}
}

@inproceedings{long2015learning,
  title={Learning transferable features with deep adaptation networks},
  author={Long, M. and Cao, Y. and Wang, J. and Jordan, M.},
  booktitle={ICML 2015}
}

@inproceedings{yu2019accelerating,
  title={Accelerating deep unsupervised DA with transfer channel pruning},
  author={Yu, C. and Wang, J. and Chen, Y. and Wu, Z.},
  booktitle={IJCNN 2019}
}

@inproceedings{hong2018conditional,
  title={Conditional generative adversarial network for structured DA},
  author={Hong, W. and Wang, Z. and Yang, M. and Yuan, J.},
  booktitle={CVPR 2018}
}

@inproceedings{bousmalis2017unsupervised,
  title={Unsupervised pixel-level DA with generative adversarial networks},
  author={Bousmalis, K. and Silberman, N. and Dohan, D. and Erhan, D. and Krishnan, D.},
  booktitle={CVPR 2017}
}

@InProceedings{pmlr-v97-peng19b,
  title = {Domain Agnostic Learning with Disentangled Representations},
  author =  {Peng, X. and Huang, Z. and Sun, X. and Saenko, K.},
  booktitle = {ICML 2019}
  }

@article{gholami2020unsupervised,
  title={Unsupervised multi-target DA: An information theoretic approach},
  author={Gholami, B. and Sahu, P. and Rudovic, O. and Bousmalis, K. and Pavlovic, V.},
  journal={IEEE Transactions on Image Processing},
  volume={29},
  pages={3993--4002},
  year={2020}
}

@inproceedings{liu2020open,
  title={Open compound DA},
  author={Liu, Z. and Miao, Z. and Pan, X. and Zhan, X. and Lin, D. and Yu, S. and Gong, B.},
  booktitle={CVPR 2020}
}

@article{gong2013reshaping,
  title={Reshaping visual datasets for DA},
  author={Gong, B. and Grauman, K. and Sha, F.},
  journal={NeurIPS 2013}
}

@article{yu2018multi,
  title={Multi-target unsupervised DA without exactly shared categories},
  author={Yu, H. and Hu, M. and Chen, S.},
  journal={arXiv 2018}
}

@article{allen2020towards,
  title={Towards Understanding Ensemble, Knowledge Distillation and Self-Distillation in Deep Learning},
  author={Allen-Zhu, Z. and Li, Y.},
  journal={arXiv 2020}
}

@article{zaras2021improving,
  title={Improving Knowledge Distillation using Unified Ensembles of Specialized Teachers},
  author={Zaras, A. and Passalis, N. and Tefas, A.},
  journal={Pattern Recognition Letters},
  volume={146},
  pages={215--221},
  year={2021}
}

@article{zhao2021similarity,
  title={Similarity Transfer for Knowledge Distillation},
  author={Zhao, H. and Gong, K. and Sun, X. and Dong, J. and Yu, H.},
  journal={arXiv 2021}
}

@article{xuan2021intra,
  title={Intra-Inter Camera Similarity for Unsupervised Person reID},
  author={Xuan, S. and Zhang, S.},
  journal={arXiv 2021},
}

@inproceedings{yu2019unsupervised,
  title={Unsupervised person reID by soft multilabel learning},
  author={Yu, H.X. and Zheng, W.S. and Wu, A. and Guo, X. and Gong, S. and Lai, J.H.},
  booktitle={CVPR 2019}
}



@inproceedings{zheng2015scalable,
  title={Scalable person reID: A benchmark},
  author={Zheng, L. and Shen, L. and Tian, L. and Wang, S. and Wang, J. and Tian, Q.},
  booktitle={ICCV 2015}
}


@article{ekladious2020dual,
  title={Dual-triplet metric learning for unsupervised DA in video-based face recognition},
  author={Ekladious, G. and Lemoine, H. and Granger, E. and Kamali, K. and Moudache, S.},
  journal={arXiv 2020}
}

@article{ge2020selfpaced,
  title={Self-paced contrastive learning with hybrid memory for domain adaptive object re-id},
  author={Ge, Y. and Zhu, F. and Chen, D. and Zhao, R. and others},
  journal={NeurIPS 2020}
}


@inproceedings{ester1996density,
  title={A density-based algorithm for discovering clusters in large spatial databases with noise},
  author={Ester, M. and Kriegel, H.P. and Sander, J. and Xu, X. and others},
  booktitle={kdd},
  volume={96},
  number={34},
  year={1996}
}

@article{nguyen2021incremental,
  title={Incremental Multi-Target DA for Object Detection with Efficient Domain Transfer},
  author={Nguyen-Meidine, L.T. and Kiran, M. and Pedersoli, M. and Dolz, J. and Blais-Morin, L.A. and Granger, E.},
  journal={arXiv 2021}
}

@inproceedings{le2020unsupervised,
  title={Unsupervised multi-target DA through knowledge distillation},
  author={Nguyen-Meidine, L.T. and Belal, A. and Kiran, M. and Dolz, J. and Blais-Morin, L.A. and Granger, E.},
  booktitle={WACV 2021}
}

@article{wei2020incremental,
  title={Incremental learning based multi-DA for object detection},
  author={Wei, X. and Liu, S. and Xiang, Y. and Duan, Z. and Zhao, C. and Lu, Y.},
  journal={Knowledge-Based Systems},
  volume={210},
  pages={106420},
  year={2020}
}

@inproceedings{li2014cuhk03,
  title={Deepreid: Deep filter pairing neural network for person reID},
  author={Li, Wei and Zhao, Rui and Xiao, Tong and Wang, Xiaogang},
  booktitle={CVPR 2014}
}

@inproceedings{wei2018msmt17,
  title={Person transfer gan to bridge domain gap for person reID},
  author={Wei, L. and Zhang, S. and Gao, W. and Tian, Q.},
  booktitle={CVPR 2018}
}

@inproceedings{isobe2021multi,
  title={Multi-target DA with collaborative consistency learning},
  author={Isobe, T. and Jia, X. and Chen, S. and He, J. and Shi, Y. and Liu, J. and Lu, H. and Wang, S.},
  booktitle={CVPR 2021}
}

@inproceedings{wu2019distilled,
  title={Distilled person reID: Towards a more scalable system},
  author={Wu, A. and Zheng, W.S. and Guo, X. and Lai, J.H.},
  booktitle={CVPR 2019}
}

@InProceedings{Nguyen-Meidine_2021_WACV,
    author    = {Nguyen-Meidine, L.T. and Belal, A. and Kiran, M. and Dolz, J. and Blais-Morin, L.A. and Granger, E.},
    title     = {Unsupervised Multi-Target DA Through Knowledge Distillation},
    booktitle = {WACV 2021}
}

@inproceedings{zhou2019omni,
  title={Omni-scale feature learning for person reID},
  author={Zhou, K. and Yang, Y. and Cavallaro, A. and Xiang, T.},
  booktitle={ICCV 2019}
}

@article{felzenszwalb2009object,
  title={Object detection with discriminatively trained part-based models},
  author={Felzenszwalb, P. and Girshick, R. and McAllester, D. and Ramanan, D.},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={32},
  number={9},
  pages={1627--1645},
  year={2009},
}

% Multi Target UDA ReID
@article{tian2021camera,
  title={A Camera Identity-guided Distribution Consistency Method for Unsupervised Multi-target Domain Person reID},
  author={Tian, J. and Tang, Q. and Li, R. and Teng, Z. and Zhang, B. and Fan, J.},
  journal={ACM Transactions on Intelligent Systems and Technology},
  volume={12},
  number={4},
  pages={1--18},
  year={2021}
  }

@article{zhong2019invariance,
      title={Invariance Matters: Exemplar Memory for Domain Adaptive Person reID}, 
      author={Zhun Z. and Liang Z. and Zhiming L. and Shaozi L. and Yi Y.},
      journal={arXiv 2019}
}

@article{he2020momentum,
      title={Momentum Contrast for Unsupervised Visual Representation Learning}, 
      author={Kaiming H. and Haoqi F. and Yuxin W. and Saining X. and Girshick, R.},
      journal={arXiv 2020}
}

@inproceedings{khurana2021unsupervised,
  title={Unsupervised DA for speech recognition via uncertainty driven self-training},
  author={Khurana, S. and Moritz, N. and Hori, T. and Le Roux, J.},
  booktitle={ICASSP 2021}
}

@inproceedings{NEURIPS2018_c5ab0bc6,
 author = {Ge, Y. and Li, Z. and Zhao, H. and Yin, G. and Yi, S. and Wang, X. and Li, H.},
 title = {FD-GAN: Pose-guided Feature Distilling GAN for Robust Person reID},
 booktitle = {NeurIPS 2018}
}

@InProceedings{Wu_2019_CVPR,
author = {Wu, A. and Zheng, W.S. and Guo, X. and Lai, J.H.},
title = {Distilled Person reID: Towards a More Scalable System},
booktitle = {CVPR 2019}
}

@inproceedings{boudiaf2020unifying,
  title={A unifying mutual information view of metric learning: cross-entropy vs. pairwise losses},
  author={Boudiaf, M. and Rony, J. and Ziko, I.M. and Granger, E. and Pedersoli, M. and Piantanida, P. and Ben Ayed, I.},
  booktitle={ECCV 2020}
}

@article{gholami2018unsupervised,
  title={Unsupervised multi-target DA: An information theoretic approach},
  author={Gholami, B. and Sahu, P. and Rudovic, O. and Bousmalis, K. and Pavlovic, V.},
  journal={IEEE Transactions on Image Processing},
  volume={29},
  pages={3993--4002},
  year={2020},
}

@inproceedings{chen2019blendingtarget,
  title={Blending-target DA by adversarial meta-adaptation networks},
  author={Chen, Z. and Zhuang, J. and Liang, X. and Lin, L.},
  booktitle={CVPR 2019}
}

@inproceedings{peng2019moment,
  title={Moment matching for multi-source DA},
  author={Peng, X. and Bai, Q. and Xia, X. and Huang, Z. and Saenko, K. and Wang, B.},
  booktitle={ICCV 2019}
}

@inproceedings{pei2018multiadversarial,
  title={Multi-adversarial DA},
  author={Z. Pei and Z. Cao and M. Long and J. Wang},
  booktitle={AAAI 2018}
}

@article{he2020multi,
  title={Multi-target multi-camera tracking by tracklet-to-target assignment},
  author={He, Y. and Wei, X. and Hong, X. and Shi, W. and Gong, Y.},
  journal={IEEE Transactions on Image Processing},
  volume={29},
  pages={5191--5205},
  year={2020},
}

@article{wen2017multi,
  title={Multi-camera multi-target tracking with space-time-view hyper-graph},
  author={Wen, L. and Lei, Z. and Chang, M.C. and Qi, H. and Lyu, S.},
  journal={Int'l J. Computer Vision},
  volume={122},
  number={2},
  pages={313--333},
  year={2017},
}

@inproceedings{ristani2018feature,
  title={Features for multi-target multi-camera tracking and reID},
  author={Ristani, E. and Tomasi, C.},
  booktitle={CVPR 2018}
}

@article{zhang2017multi,
  title={Multi-target, multi-camera tracking by hierarchical clustering: Recent progress on dukemtmc project},
  author={Zhang, Z. and Wu, J. and Zhang, X. and Zhang, C.},
  journal={arXiv 2017}
}
